The LU-LC conjecture is false

The LU-LC conjecture is an important open problem concerning the structure of entanglement of states described in the stabilizer formalism. It states that two local unitary equivalent stabilizer states are also local Clifford equivalent. If this conjecture were true, the local equivalence of stabilizer states would be extremely easy to characterize. Unfortunately, however, based on the recent progress made by Gross and Van den Nest, we find that the conjecture is false.

==> readme <==
cegen.m is the random generator of counterexamples. To obtain a
counterexample, run it in Octave/Matlab as

> [Q,S,c] = cegen(6);

If Octave complains that `bitxor' is undefined, update your Octave.


<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<

verify.m is a verifier we wrote. Call it as

> verify(6,Q,S,c);


<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<

counterexample saves the example we used in the paper.
It is Octave only but also human readable.


<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<

gauss4.m implements the modified Gaussian elimination method.
gauss.m implements the Gaussian elimination over F_2
solution.m generates the basis of the solution space of Ax=0 over F_2
tograph.m converts state in the quadratic form to the graph state form
lc.m checks LC equivalence of two graph states

The following commands checks the LC equivalence of
stabilizer states \ket{Q,S} and \ket{0,S}

> [Q,S,c] = cegen(6); lc(tograph(Q,S), tograph(zeros(size(Q)), S));

